Enhancing Heterogeneous Federated Learning with Knowledge Extraction and Multi-Model Fusion

Concerned with user data privacy, this paper presents a new federated learning (FL) method that trains machine learning models on edge devices without accessing sensitive data. Traditional FL methods, although privacy-protective, fail to manage model heterogeneity and incur high communication costs due to their reliance on aggregation methods. To address this limitation, we propose a resource-aware FL method that aggregates local knowledge from edge models and distills it into robust global knowledge through knowledge distillation. This method allows efficient multi-model knowledge fusion and the deployment of resource-aware models while preserving model heterogeneity. Our method improves communication cost and performance in heterogeneous data and models compared to existing FL algorithms. Notably, it reduces the communication cost of ResNet-32 by up to 50\% and VGG-11 by up to 10$\times$ while delivering superior performance.

==> content/02_motivation.tex <==
\section{Motivation – Use Cases}
\label{sec:motivation}

The rapid increase of computational power on mobile and embedded devices has enabled the training of more and more applications on the edge. Edge devices are becoming more powerful, so many machine learning (ML) tasks can be performed directly on edge devices instead of using high-end systems. However, deploying ML models on edge devices requires certain considerations such as storage, computational cost, and privacy. In particular, large-scale ML models (e.g., DNNs) are difficult to deploy on resource-limited edge devices \cite{imteaj2022iot,nguyen2021iot} and it makes no sense to apply large-scale ML to devices with weak computing power. On the other hand, the aggregating efficiency and quality on the server side are  important for FL settings. First, decentralized training on edge devices requires more training epochs than centralized training, and data heterogeneity is a major problem in decentralized model training \cite{zhang2021adaptive_noniid}. Second, the frequent sharing of model weights between edge devices and central servers incurs high communication costs. Third, simple aggregating of local models has the potential issues of over-fitting and high variance in prediction. Therefore, fast edge computing and efficient server inference is demanded by modern FL applications. In light of the prevailing trends in edge computing, and the aforementioned FL requirements, we are motivated to design a multi-model fusion of knowledge from resource-aware edge-trained tiny-size neural networks.

%With advancements in the performance of mobile and embedded devices, more and more applications are moving to the edge. Improved ML models and advanced weight pruning techniques mean a significant amount of future ML workload will come from training and  inference on edge devices~\cite{park2018dl_inference_fb}. Edge devices operate under strict performance, power, and privacy constraints, which are affected by factors such as model size and accuracy, training and inference time, and privacy requirements. 

%Therefore, the prevailing edge computing trend alongside FL requirements and edge constraints motivates  us to address challenges in HPC.
% An HPC scenario where data communication cost is important. (Claim 1 in the introduction)
%Firstly, frequent sharing of model weights between edge devices and the central server incurs a hefty communication cost~\cite{problemsfl,Sheller2018medical}. Thus, reducing communication overhead is imperative. 
% An HPC/Edge scenario where resources are limited so knowledge transfer should help (Claim 2)
%Secondly, the increasing demand for computing, memory, and storage for AI models (e.g., deep neural networks -- DNNs) makes it hard to deploy them on resource-constrained Internet-of-Things~(IoT) and edge devices~\cite{imteaj2022iot,nguyen2021iot}. Transfer learning can be a viable solution to address this problem.
% a clustering-based federated energy demand learning approach is implemented~\cite{saputra2019energy_ev} for electric vehicle networks to make
% energy demand prediction
% An HPC scenario where we need inference time to be fast. (Claim 3)
%Thirdly, latency-sensitive applications with privacy constraints (e.g., self-driving cars~\cite{kato2018auto}, augmented reality~\cite{mangiante2017vr}) in particular, are better suited for fast edge computing~\cite{wu2019ml_fb}. Hence, cutting back on inference time is quite important.
% An HPC scenario where we need scalability (Claim 5)

Federated learning has already shown its potential in practical applications, including health care \cite{healthcare}, environment protection \cite{environment}, electrical vehicles \cite{electricvehicle}, etc. 
Google, Apple, and NVIDIA are using FL for their applications nowadays (e.g., Google Keyboard~\cite{yang2018keyboard,chen2019keyboard}, Apple Siri~\cite{apple2019siri,paulik2021siri}, NVIDIA medical imaging~\cite{li2019nvidia}) In consequence, designing efficient FL models and deploying them effectively and fairly on edge devices is crucial for improving the performance of edge computing in the future.

%thanks to their large number of edge devices. Hence, scalability is important in FL and HPC settings.
% imbalance/non-IID dataset on edge:
%Lastly, training data on client edge devices depends on the user's unique usage causing an overall non-IID~\cite{mcmahan2017fedavg,zhao2018federated} user dataset. Data heterogeneity is a major problem in decentralized model training~\cite{problemsfl,nishio2019clientselection,zhao2018federated,hsieh2020quagmire,li2020convergence_noniid,lim2020federated,li2020fedprox,reddi2021fedopt,karimireddy2020scaffold,wang2020fednova,zhang2021adaptive_noniid}.

==> content/figtex/f_ablation.tex <==
\begin{figure*}
 \begin{center}

\centerline{\includegraphics[width=1.0\linewidth]{content/Figures/ablation.pdf}}
\caption{\proj under different FL settings. $N$ is the total number of clients, $f$ is the client sample ratio.  The model type is the network at local devices. The knowledge network is ResNet-20 in all cases for \proj.}
\vspace{-1em}
\label{fig:ablation}
\end{center}
 \end{figure*}

==> content/figtex/f_converged_round.tex <==
\begin{figure}
 \begin{center}

\centerline{\includegraphics[width=1.0\linewidth]{content/Figures/converged_round.pdf}}
\caption{Comparison of \proj with SoTAs: the communication rounds need to read 50\% top-1 accuracy. Different communication rounds correspond to different local epochs.}
\vspace{-1em}
\label{fig:converged_rounds}
\end{center}
 \end{figure}

==> content/figtex/f_data_distri.tex <==
\begin{figure*}
 \begin{center}

\centerline{\includegraphics[width=1.0\linewidth]{content/Figures/heat_map_plt.pdf}}
\caption{Heterogeneous distribution of CIFAR-10 in each client. The color bar is used to indicate the number of data samples, and each rectangle represents the number of data samples of a particular class that is assigned to a specific client.}
% \vspace{-1em}
\label{fig:data_distri}
\end{center}
 \end{figure*}


==> content/figtex/f_round_target_acc.tex <==
\begin{figure}
 \begin{center}
%  \vskip -0.4in

\centerline{\includegraphics[width=1.0\linewidth]{content/Figures/round_target_acc.pdf}}
% \centerline{\includegraphics[width=\linewidth]{figure/train_effi_2.pdf}}
\caption{Communication rounds to achieve target accuracy. The lower the better.}
\vspace{-1em}
\label{fig:com_acc}
\end{center}
 \end{figure}

==> content/tbtex/t_com_convergence.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\caption{Comparison of communication cost with SoTAs to achieve model convergence.}
\label{tab:com_converge}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllll}
\hline
\multirow{2}{*}{Method}  & \multirow{2}{*}{Clients} & \multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Sample\\ Ratio\end{tabular}} & \multirow{2}{*}{Converge Rounds} & \multicolumn{3}{l}{Communication Cost} & \multirow{2}{*}{Converge Acc.} & \multirow{2}{*}{$\Delta$ Acc.} \\
                         &                          &                        &                                                                         &                                  & Round/Client   & Total   & Speedup     &                                &                                \\ \hline
\multirow{7}{*}{FedAvg}  & \multirow{3}{*}{30}      & ResNet-20              & 0.4                                                                     & 163                              & 2.1MB          &  4.01GB       & (1 $\times$)  & 64.95\%                        & 0\%                            \\
                         &                          & ResNet-32              & 0.4                                                                     & 182                              & 3.2MB          & 6.83GB        & (1 $\times$)  & 64.92\%                        & 0\%                            \\
                         &                          & VGG-11                 & 0.4                                                                     & 163                              & 42MB           & 80.23GB        & (1 $\times$)  & 64.69\%                        & 0\%                            \\ \cline{2-10} 
                         & \multirow{2}{*}{50}      & ResNet-20              & 0.7                                                                     & 195                              & 2.1MB          & 14.00GB        & (1 $\times$)  & 33.22\%                        & 0\%                            \\
                         &                          & ResNet-32              & 0.7                                                                     & 195                              & 3.2MB          &  21.33GB       & (1 $\times$)  & 33.19\%                        & 0\%                            \\ \cline{2-10} 
                         & \multirow{2}{*}{100}     & ResNet-20              & 0.5                                                                     & 111                              & 2.1MB          &  11.38GB       & (1 $\times$)  & 61.39\%                        & 0\%                            \\
                         &                          & ResNet-32              & 0.5                                                                     & 122                              & 3.2MB          & 19.06GB        & (1 $\times$)  & 61.38\%                        & 0\%                            \\ \hline
\multirow{7}{*}{FedNova} & \multirow{3}{*}{30}      & ResNet-20              & 0.4                                                                     & 195                              & 4.2MB          &   9.60GB      & (0.42 $\times$)  & 69.28\%                        &  +4.33\%                              \\
                         &                          & ResNet-32              & 0.4                                                                     & 196                              & 6.4MB          & 14.70GB        & (0.46 $\times$)  & 69.13\%                        &    +4.21\%                            \\
                         &                          & VGG-11                 & 0.4                                                                     & 196                              & 84MB           & 192.94GB        & (0.42 $\times$)  & 69.15\%                        &     +4.46\%                           \\ \cline{2-10} 
                         & \multirow{2}{*}{50}      & ResNet-20              & 0.7                                                                     & 167                              & 4.2MB          & 23.97GB        & (0.58 $\times$)  & 31.27\%                        &         -1.95\%                       \\
                         &                          & ResNet-32              & 0.7                                                                     & 183                              & 6.4MB          & 40.03GB        & (0.53 $\times$)  & 31.87\%                        &            -1.32\%                    \\ \cline{2-10} 
                         & \multirow{2}{*}{100}     & ResNet-20              & 0.5                                                                     & 191                              & 4.2MB          & 39.17GB        & (0.29 $\times$)  & 68.30\%                        &     +6.91\%                           \\
                         &                          & ResNet-32              & 0.5                                                                     & 192                              & 6.4MB          &  60.00GB       & (0.32 $\times$)  & 67.27\%                        &           +5.89\%                     \\ \hline
\multirow{7}{*}{FedProx} & \multirow{3}{*}{30}      & ResNet-20              & 0.4                                                                     & 163                              & 2.1MB          &    4.01GB     &    (1 $\times$)         & 64.00\%                        &              -0.95\%                  \\
                         &                          & ResNet-32              & 0.4                                                                     & 195                              & 3.2MB          &  7.31GB        &     (0.93 $\times$)        & 64.75\%                        &      -0.17\%                          \\
                         &                          & VGG-11                 & 0.4                                                                     & 188                              & 42MB           &  92.53GB       &     (0.87 $\times$)        & 64.13\%                        &     -0.56\%                           \\ \cline{2-10} 
                         & \multirow{2}{*}{50}      & ResNet-20              & 0.7                                                                     & 195                              & 2.1MB          & 14.00GB        &      (1 $\times$)       & 32.43\%                        &  -0.79\%                              \\
                         &                          & ResNet-32              & 0.7                                                                     & 195                              & 3.2MB          & 21.33GB        &     (1 $\times$)        & 32.89\%                        &    -0.3\%                            \\ \cline{2-10} 
                         & \multirow{2}{*}{100}     & ResNet-20              & 0.5                                                                     & 118                              & 2.1MB          &   12.10GB      &     (0.94 $\times$)        & 62.55\%                        &    +1.16\%                            \\
                         &                          & ResNet-32              & 0.5                                                                     & 128                              & 3.2MB          & 20.00GB        &    (0.95 $\times$)         & 63.69\%                        &    +2.31\%                            \\ \hline
\multirow{7}{*}{FedKEMF} & \multirow{3}{*}{30}      & ResNet-20              & 0.4                                                                     & 193                              & 2.1MB          &   4.75GB      &     (0.84 $\times$)        & 73.35\%                        &              +8.40\%                  \\
                         &                          & ResNet-32              & 0.4                                                                     & 199                              & 2.1MB          & 4.90GB         &    (1.39 $\times$)         & 72.47\%                        &     +7.55\%                           \\
                         &                          & VGG-11                 & 0.4                                                                     &  191                                & 2.1MB          & 4.70GB        &     (17.07 $\times$)        &     74.58\%                           &   +9.89\%                             \\ \cline{2-10} 
                         & \multirow{2}{*}{50}      & ResNet-20              & 0.7                                                                     & 199                              & 2.1MB          & 14.28GB        &    (0.98 $\times$)         & 57.92\%                        &  +24.70\%                              \\
                         &                          & ResNet-32              & 0.7                                                                     & 197                              & 2.1MB          &  14.14GB       &     (1.51 $\times$)        & 71.87\%                        &     +38.68\%                           \\ \cline{2-10} 
                         & \multirow{2}{*}{100}     & ResNet-20              & 0.5                                                                     & 127                              & 2.1MB          & 13.02GB         &    (0.87 $\times$)         & 68.78\%                        &   +7.39\%                             \\
                         &                          & ResNet-32              & 0.5                                                                     & 175                              & 2.1MB          & 17.94GB        &    (1.06 $\times$)         & 72.01\%                        &    +10.63\%                            \\ \hline
\end{tabular}%
}
\end{table*}

==> content/tbtex/t_com_target.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t]
\centering
\caption{Comparison of communication cost with SoTAs to achieve target accuracy. The model marked with `*' failed to achieve target accuracy.}
\label{tab:com_target}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{Method}  & \multirow{2}{*}{Model} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Target \\ Accuracy\end{tabular}} & \multirow{2}{*}{Clients} & \multirow{2}{*}{Communication Rounds} & \multirow{2}{*}{Round/Client} & \multicolumn{2}{c}{Communication Cost} & \multirow{2}{*}{Speed Up} \\
                         &                        &                                                                             &                          &                                       &                               & Total          & $\Delta$ Cost         &                           \\ \hline
\multirow{7}{*}{FedAvg}  & ResNet-20              & \multirow{3}{*}{65\%}                                                       & \multirow{3}{*}{30}      & 163                                   & 2.1MB                         &     4.01GB           & 0GB                   & (1 $\times$)              \\
                         & ResNet-32              &                                                                             &                          & 183                                   & 3.2MB                         &     6.86GB           & 0GB                   & (1 $\times$)              \\
                         & VGG-11                 &                                                                             &                          & 166                                   & 42MB                          &   81.70GB             & 0GB                   & (1 $\times$)              \\ \cline{2-9} 
                         & ResNet-20$^*$          & \multirow{2}{*}{57\%}                                                       & \multirow{2}{*}{50}      & 400                                   & 2.1MB                         &   28.71GB             & 0GB                   & (1 $\times$)              \\
                         & ResNet-32$^*$          &                                                                             &                          & 400                                   & 3.2MB                         &     43.75GB           & 0GB                   & (1 $\times$)              \\ \cline{2-9} 
                         & ResNet-20              & \multirow{2}{*}{60\%}                                                       & \multirow{2}{*}{100}     & 109                                   & 2.1MB                         &     11.18GB           & 0GB                   & (1 $\times$)              \\
                         & ResNet-32              &                                                                             &                          & 109                                   & 3.2MB                         &    17.03GB            & 0GB                   & (1 $\times$)              \\ \hline
\multirow{7}{*}{FedNova} & ResNet-20              & \multirow{3}{*}{65\%}                                                       & \multirow{3}{*}{30}      & 147                                   & 4.2MB                         &     7.24GB           &  +3.22GB                      &    (0.55 $\times$)                     \\
                         & ResNet-32              &                                                                             &                          & 147                                   & 6.4MB                         &    11.03GB            & +4.16GB                      &       (0.62 $\times$)                    \\
                         & VGG-11                 &                                                                             &                          & 166                                   & 84MB                          & 163.41GB               &      +81.70GB                 &         (0.50 $\times$)                   \\ \cline{2-9} 
                         & ResNet-20$^*$          & \multirow{2}{*}{57\%}                                                       & \multirow{2}{*}{50}      & 400                                   & 4.2MB                         &  57.42GB              &            +28.71GB           & (0.50 $\times$)                            \\
                         & ResNet-32$^*$          &                                                                             &                          & 400                                   & 6.4MB                         &    87.50GB            &    +43.75GB                   &  (0.50 $\times$)                          \\ \cline{2-9} 
                         & ResNet-20              & \multirow{2}{*}{60\%}                                                       & \multirow{2}{*}{100}     & 182                                   & 4.2MB                         &    37.32GB            &   +26.15GB                    &               (0.30 $\times$)             \\
                         & ResNet-32              &                                                                             &                          & 155                                   & 6.4MB                         &   48.44GB             &    +31.41GB                   &                 (0.35 $\times$)           \\ \hline
\multirow{7}{*}{FedProx} & ResNet-20              & \multirow{3}{*}{65\%}                                                       & \multirow{3}{*}{30}      & 200                                   & 2.1MB                         &   4.92GB             &   +0.91GB                    &       (0.82 $\times$)                     \\
                         & ResNet-32              &                                                                             &                          & 195                                   & 3.2MB                         &  7.31GB              &         +0.45GB              &  (0.94 $\times$)                          \\
                         & VGG-11                 &                                                                             &                          & 200                                   & 42MB                          &  98.44GB              &      +16.73GB               & (0.83 $\times$)                           \\ \cline{2-9} 
                         & ResNet-20$^*$          & \multirow{2}{*}{57\%}                                                       & \multirow{2}{*}{50}      & 400                                   & 2.1MB                         &   28.71GB             &  0GB                     &    (1 $\times$)                        \\
                         & ResNet-32$^*$          &                                                                             &                          & 400                                   & 3.2MB                         &    43.75GB            &   0GB                    &    (1 $\times$)                        \\ \cline{2-9} 
                         & ResNet-20              & \multirow{2}{*}{60\%}                                                       & \multirow{2}{*}{100}     & 109                                   & 2.1MB                         &   11.18GB             &    0GB                   &  (1 $\times$)                          \\
                         & ResNet-32              &                                                                             &                          & 109                                   & 3.2MB                         &   17.03GB             &    0GB                   & (1 $\times$)                           \\ \hline
\multirow{7}{*}{FedKEMF } & ResNet-20              & \multirow{3}{*}{65\%}                                                       & \multirow{3}{*}{30}      & 76                                    & 2.1MB                         &  1.87GB              &    -2.14GB                   &       (2.14 $\times$)                     \\
                         & ResNet-32              &                                                                             &                          & 87                                    & 2.1MB                         &    2.14GB            &              -4.72GB         &  (3.21 $\times$)                          \\
                         & VGG-11                 &                                                                             &                          &  65                                     & 2.1MB                          &     1.60GB           &   -80.10GB                    &    (51.08 $\times$)                        \\ \cline{2-9} 
                         & ResNet-20              & \multirow{2}{*}{57\%}                                                       & \multirow{2}{*}{50}      & 188                                   & 2.1MB                         &  13.49GB              &     -15.22GB                  &   (2.13 $\times$)                         \\
                         & ResNet-32              &                                                                             &                          & 40                                   & 2.1MB                         &  2.87GB              &     -40.88GB                  &       (15.24 $\times$)                     \\ \cline{2-9} 
                         & ResNet-20              & \multirow{2}{*}{60\%}                                                       & \multirow{2}{*}{100}     & 53                                    & 2.1MB                         &  5.43GB              &       -5.74GB                & (2.06 $\times$)                           \\
                         & ResNet-32              &                                                                             &                          & 45                                    & 2.1MB                         &  4.61GB              &    -12.42GB                   &   (3.69 $\times$)                         \\ \hline
\end{tabular}%
}
\end{table*}

==> content/tbtex/t_model_stat.tex <==
\begin{table*}
\centering
\caption{Models statistics in CIFAR-10 datatset.}
\label{tab:model_stat}
\begin{tabular}{cccc}
\hline
 & \textbf{Model size (Mb)} & \textbf{\# of parameters (Thousands)} & \textbf{Computational cost (MMACs)} \\ \hline
VGG-11       & 21  & 9,750  & 153.72 \\
ResNet-20    & 1.05 & 269.72 & 40.93  \\
ResNet-32    & 1.6 & 464.15 & 69.47  \\
ResNet-44    & 2.7 & 658.59 & 98.01  \\
\hline
% MobileNet    & 13  & 3,220  & 47.18  \\
% EfficientNet & 14  & 3,600  & 31.43  \\ 
\end{tabular}
\end{table*}
